A Prolog Program for Bottom-up Evaluation

This short paper describes a simple and intuitive Prolog program, a metainterpreter, that computes the bottom up meaning of a simple positive Horn clause definition. It involves a simple transformation of the object program rules into metarules, which are then used by a metainterpreter to compute bottom up the model of the original program. The resulting algorithm is a form of semi-naive bottom-up evaluation. We discuss various reasons why this Prolog program is particularly interesting. In particular, this is perhaps the only Prolog program for which I find the use of Prolog's assert/1 to be intrinsic, easily understood, and the best, most perspicuous, way to program an algorithm. This short paper might be best characterized as a Prolog programming pearl.

==> eptcsdata.tex <==
\providecommand{\firstpage}{229}
\providecommand{\publicationstatus}{P. Cabalar, F. Fabiano, M. Gebser, G. Gupta and Th. Swift (Eds.):\\ 40th International Conference on Logic Programming (ICLP 2024)\\
EPTCS 416, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.416.20}{10.4204/EPTCS.416.20}}

